Quasi periodic oscillations in black hole binaries

Fast time variability is the most prominent characteristic of accreting systems and the presence of quasi periodic oscillations (QPOs) is a constant in all accreting systems, from cataclysmic variables to AGNs, passing through black hole and neutron star X-ray binaries and through the enigmatic ultra-luminous X-ray sources. In this paper I will briefly review the current knowledge of QPOs in black hole X-ray binaries, mainly focussing on their observed properties, but also mentioning the most important models that have been proposed to explain the origin of QPOs over the last decades.

==> definitions.tex <==
\newcommand{\he}[1] {He\,{\sc #1}}
\newcommand{\hel}[2] {He\,{\sc #1}~$\lambda$#2}
\newcommand{\ha}{H$\alpha$}
\newcommand{\hb}{H$\beta$}
\newcommand{\hg}{H$\gamma$}
\newcommand{\hd}{H$\beta$}
\newcommand{\hep}{H$\epsilon$}
\newcommand{\ionl}[3] {#1\,{\sc #2}~$\lambda$#3}
\newcommand{\ion}[2] {#1\,{\sc #2}}
%
% de aapp4
%
\def\kms{\mbox{${\rm km}\:{\rm s}^{-1}\:$}}
\def\ms{${\rm m}\:{\rm s}^{-1}\:$}

\def\lesssim{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$<$}}}}
\let\la=\lesssim
\def\gtrsim{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$>$}}}}
\let\ga=\gtrsim
\def\fdg{\hbox{$.\!\!^\circ$}}
\newcommand{\fdeg}{\hbox{$.\!\!^\circ$}}
\def\farcs{\hbox{$.\!\!^{\prime\prime}$}}
\def\arcsec{\hbox{$^{\prime\prime}$}}
\def\kmm{${\rm km}^{-1}$}
\def\d{{\rm d}}
\def\degree{\mbox{$^{\circ}$}}
\def\sol{~\mathrm{M}_\odot}
\def\lx{L_\mathrm{X}}
\def\kem{K_\mathrm{em}}
